In-Situ Mode: Generative AI-Driven Characters Transforming Art Engagement Through Anthropomorphic Narratives

Art appreciation serves as a crucial medium for emotional communication and sociocultural dialogue. In the digital era, fostering deep user engagement on online art appreciation platforms remains a challenge. Leveraging generative AI technologies, we present EyeSee, a system designed to engage users through anthropomorphic characters. We implemented and evaluated three modes (Narrator, Artist, and In-Situ) acting as a third-person narrator, a first-person creator, and first-person created objects, respectively, across two sessions: Narrative and Recommendation. We conducted a within-subject study with 24 participants. In the Narrative session, we found that the In-Situ and Artist modes had higher aesthetic appeal than the Narrator mode, although the Artist mode showed lower perceived usability. Additionally, from the Narrative to Recommendation session, we found that user-perceived relatability and believability within each interaction mode were sustained, but the user-perceived consistency and stereotypicality changed. Our findings suggest novel implications for applying anthropomorphic in-situ narratives to other educational settings.

==> SECTIONS/3.ResearchQuestion.tex <==
\section{RESEARCH QUESTIONS}

Based on the existing literature and identified research gaps, we aim to explore the following research questions:

\textbf{[RQ1]} How do users \underline{perceive} engagement level and \underline{interact} with the different characters? 

%--- This can be answered by comparing the first narration task’s scales and log among the three conditions. 

%\andrea{maybe? RQ1.5: what correlates with the users' evaluations? (IV: engagements; DV: six dimensions}

\textbf{[RQ2]} How do users \underline{perceive} the characters and what engagement factors in their interactions are \underline{associated} with this perception?

%How do users \underline{perceive} the characters and the \underline{effect} of their interactions with them in the EyeSee system?

%What's the \underline{effect} of perception using different EyeSee characters on satisfaction and trust with artworks recommended by characters?

%--- This can be answered by comparing the 2nd recommendation task’s scales among the three conditions.

% \textbf{[RQ3]} How do people \underline{choose} EyeSee characters to interact with different artworks?

% --- this can be answered by the 3nd free-will task’s interaction logs









==> SECTIONS/6.1.Finding1.tex <==


  






==> SECTIONS/6.2.Finding2.tex <==





